MonoPlane: Exploiting Monocular Geometric Cues for Generalizable 3D Plane Reconstruction

This paper presents a generalizable 3D plane detection and reconstruction framework named MonoPlane. Unlike previous robust estimator-based works (which require multiple images or RGB-D input) and learning-based works (which suffer from domain shift), MonoPlane combines the best of two worlds and establishes a plane reconstruction pipeline based on monocular geometric cues, resulting in accurate, robust and scalable 3D plane detection and reconstruction in the wild. Specifically, we first leverage large-scale pre-trained neural networks to obtain the depth and surface normals from a single image. These monocular geometric cues are then incorporated into a proximity-guided RANSAC framework to sequentially fit each plane instance. We exploit effective 3D point proximity and model such proximity via a graph within RANSAC to guide the plane fitting from noisy monocular depths, followed by image-level multi-plane joint optimization to improve the consistency among all plane instances. We further design a simple but effective pipeline to extend this single-view solution to sparse-view 3D plane reconstruction. Extensive experiments on a list of datasets demonstrate our superior zero-shot generalizability over baselines, achieving state-of-the-art plane reconstruction performance in a transferring setting. Our code is available at https://github.com/thuzhaowang/MonoPlane .

==> tables/table_matteport_single.tex <==
\begin{table}[]
\caption{Single-view plane reconstruction evaluation on Matterport3D~\cite{chang2017matterport3d}.}
\centering
\begin{tabular}{lllllll}
\toprule
\centering
\multirow{2}{*}{Method / Metrics} & \multicolumn{3}{c}{Plane Segmentation Metrics} & \multicolumn{3}{c}{Per-plane Recall (depth)} \\ \cmidrule(r){2-7} 
                                  & VOI~(↓)   & RI~(↑)  & \multicolumn{1}{l}{SC~(↑)}  & @0.05m     & @0.1m   & @0.6m    \\
\midrule 
\multicolumn{7}{c}{Matterport3D~\cite{chang2017matterport3d}} \\
\midrule
PlaneRCNN~\cite{liu2019planercnn} & 1.826 & 0.837 & 0.585 &  0.023 & 0.082 & 0.388\\
PlaneTR~\cite{tan2021planetr}  & 1.553 & 0.846  & 0.610  &  0.019 & 0.056 & 0.223\\
Ours  & 1.222  &   0.902   & 0.700   &   0.084   &  0.210  &  0.502\\
\bottomrule
\end{tabular}
\label{tab::singleview-matterport}
\end{table}

==> tables/table_scannet_single.tex <==
\begin{table}[]
%We do not evaluate plane detection for PlaneRecover~\cite{yang2018recovering} since their method does not estimate a per-pixel depth map for the whole image.}
\centering
\caption{Single-view evaluation on ScanNet~\cite{dai2017scannet}. Note that all of the compared methods are trained on ScanNet except for ours.}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lllllll}
\toprule
\centering
\multirow{2}{*}{Method / Metrics} & \multicolumn{3}{c}{Plane Segmentation Metrics} & \multicolumn{3}{c}{Plane Recall (depth)} \\ \cmidrule(r){2-7} 
                                  & VOI~(↓)   & RI~(↑)  & \multicolumn{1}{l}{SC~(↑)}  & @0.05m     & @0.1m   & @0.6m   \\ 
%\midrule
%PlaneRCNN~(ScanNet)~\cite{liu2019planercnn} & 1.297 & 0.852 & 0.699 &  0.194 & 0.417 & 0.674\\
%PlaneTR~(ScanNet)~\cite{tan2021planetr}  & 0.767 & 0.925 & 0.838 & 0.245 & 0.437 & 0.616\\
%PlaneRecTR~(ScanNet, SSA)~\cite{shi2023planerectr} & 0.652 & 0.943 & 0.865  & 0.363 & 0.577 & 0.756 \\ 
%PlaneRecover~(Synthia, SSA) ~\cite{yang2018recovering} & 2.517 & 0.639  & 0.400 &  - & - & -\\
%Ours~(SSA)  &   1.172  &   0.878 & 0.724  & 0.223  &  0.435  &  0.640 \\
\midrule
PlaneRCNN~(ScanNet)~\cite{liu2019planercnn} & 1.297 & 0.852 & 0.699 &  0.188 & 0.388 & 0.668\\
PlaneTR~(ScanNet)~\cite{tan2021planetr} & 0.761 & 0.923  & 0.837 & 0.272 & 0.455 & 0.614 \\
PlaneRecTR~(ScanNet)~\cite{shi2023planerectr} & \textbf{0.652} & \textbf{0.943} & \textbf{0.865} & \textbf{0.345} & \textbf{0.548} & \textbf{0.753} \\ 
\midrule
Ours~(Omnidata) & 0.910 & 0.912 & 0.798 & 0.214 & 0.424 & 0.662 \\ 
Ours~(ZeroDepth) & 1.048 & 0.889 & 0.756 & 0.118 & 0.297 & 0.606 \\
%\midrule
%PlaneTR~(ScanNet, Metric)~\cite{tan2021planetr} & 0.761 & 0.923  & 0.837 & 0.208 & 0.382 & 0.614 \\
%PlaneRCNN~(ScanNet, Metric)~\cite{liu2019planercnn} & 1.297 & 0.852 & 0.699 & 0.12 & 0.288 & 0.662\\
%PlaneRecTR~(ScanNet, Metric)~\cite{shi2023planerectr} & 0.652 & 0.943 & 0.865  & 0.232 & 0.442 & 0.754 \\ 
%Ours~(ZeroDepth, Metric)~\cite{shi2023planerectr} & 0.913 & 0.909 & 0.797 & 0.081 & 0.442 & 0.642 \\ 
\bottomrule
\end{tabular}}

\label{tab::scannet}
\end{table}
